Decision Rules for Robotic Mobile Fulfillment Systems

The Robotic Mobile Fulfillment Systems (RMFS) is a new type of robotized, parts-to-picker material handling system, designed especially for e-commerce warehouses. Robots bring movable shelves, called pods, to workstations where inventory is put on or removed from the pods. This paper simulates both the pick and replenishment process and studies the order assignment, pod selection and pod storage assignment problems by evaluating multiple decision rules per problem. The discrete event simulation uses realistic robot movements and keeps track of every unit of inventory on every pod. We analyze seven performance measures, e.g. throughput capacity and order due time, and find that the unit throughput is strongly correlated with the other performance measures. We vary the number of robots, the number of pick stations, the number of SKUs (stock keeping units), the order size and whether returns need processing or not. The decision rules for pick order assignment have a strong impact on the unit throughput rate. This is not the case for replenishment order assignment, pod selection and pod storage. Furthermore, for warehouses with a large number of SKUs, more robots are needed for a high unit throughput rate, even if the number of pods and the dimensions of the storage area remain the same. Lastly, processing return orders only affects the unit throughput rate for warehouse with a large number of SKUs and large pick orders.

==> sections/dea.tex <==
Data Envelopment Analysis (DEA) will be used to evaluate the performance of the mechanisms.
DEA is a technique from production economics (\citet{DEA.Ray}), that studies multiple so-called ``Decision Making Units'' (DMUs), where each DMU is an entity that uses inputs to produce outputs.
DEA compares multiple DMUs to examine how efficiently  the DMUs are transforming inputs into outputs, relative to each other.
The input is not constrained to be a single resource, but can be multiple different resources, and similarly for the outputs.
If both the input and the output is a single resource, then the efficiency of the DMUs can simply be compared by calculating the ratio between output and input per DMU see \citet{A727}.
The main advantage of DEA is that it can compare the performance in situations where multiple inputs and/or outputs are used, especially because DEA allows each input, and also each output, to be measured in its own units and scale.
Moreover, DEA is a parameterless method, which means that no coefficients, weights or parameters need to be estimated and no statistical distributions need to be assumed or tested for.\\
Since the three concepts of DMU, inputs and outputs is quite abstract, the technique lends itself to application in different contexts.
As detailed in \citet{A726}, DEA has been applied in tens of different disciplines, from banking and health care to agriculture and education, to name just a few.
DEA has also been used extensively in the context of logistics, a theoretical contribution would for example be \citet{A731}, who show how to apply DEA to the transportation problem.
Examples of practical applications in logistics include the airlines and the railways.
\citet{A741} and \citet{A743} were early pioneers in applying DEA to the airline industry, arguing that relying solely on financial metrics did not provide an accurate view on performance.
A recent example of applying DEA to the airline industry would be \citet{A742}, which applies a network DEA to find inefficiencies in the European airline industry.
Early examples of applying DEA to the railways include \citet{A739} and \citet{A744}.
\citet{A739} uses a two stage approach where DEA first is applied to estimate the efficiency of railways in 19 OECD countries and secondly a Tobit regression is ran using these efficiency scores.
They note that efficiency measures can only be compared when controlling for differences in the operating and market environments of the railways.
\citet{A744} compares DEA to the several other techniques and concludes that the results from DEA can be distorted by extreme values in some of the inputs.
Recently, \citet{A740} applied a network DEA to the public rail transit in the U.S.A., arguing that whereas a basic DEA is a black-box method that does not provide the reasons behind the differences in efficiencies, a network DEA does, because it includes DEA analysis of intermediate resources in between the inputs and outputs.\\
DEA has also been applied extensively to analyze the performance of warehouses, for example by \citet{A732}, \citet{A733}, \citet{A477}, \citet{A735} and \citet{A728}.
\citet{A732} look at 57 warehouses in the U.S.A. across multiple industries in the period 1993 - 1997.
They note that DEA assumes that DMUs operate under identical conditions, i.e. the homogeneity assumption, which may not hold in practice.
To control for violation of this assumption, the efficiency scores from the DEA can be regressed on environmental factors.
\citet{A732} use a logistic regression to control for warehouse size, automation level and unionization.
They conclude that smaller warehouses tend to be more efficient than smaller warehouses, that warehouses with lower levels of automation tend be more efficient than those with higher levels and that unionization is not negatively associated with efficiency.
\citet{A733} apply DEA to a group of 19 warehouses operated during 2004 by a third-party logistics (3PL) provider based in the U.S.A.
The warehouses are homogeneous, which implies that a second phase with regressions to control for environmental difference was not necessary.
Besides a basic DEA, they also apply a restricted DEA model, where the restrictions on the weights given to the inputs and outputs are provided by expert opinion.
They argue that in an unrestricted, basic DEA model, the weights given to some inputs may be so low as to be practically zero, meaning that the model effectively ignores these inputs, even though these inputs may be important to management.
One of their conclusions is that smaller warehouses tend to be more efficient than larger ones.
\citet{A477} apply DEA in a cross-sectional and longitudinal study to benchmark 65 European distribution centers in the Netherlands over the time period 2000 to 2004.
They conclude that European warehouses are more efficient than Asian and American warehouses.
Moreover, it appears that outsourced operations were more efficient than own-account operations.
However, during this time period efficiency as well as productivity deteriorated even as the level of available technology rose.
\citet{A735} focus on how to study a warehousing dataset using DEA and show a number of statistical tests that can be deployed.
The dataset they use as an illustration collected over a five year periods containing over 400 warehouses.
Managers of the warehouses themselves filled went to a website to fill in data about their warehouse. 
Since the operating environment of the warehouses can be very different, \citet{A735} also opted for a two phase procedure, where in the first phase the efficiency scores are calculated and in the second phase the efficiency scores are regressed on other variables relating to the operating conditions in the warehouse.
In addition, they include three types of tests.
The first test checks for redundancy in the inputs and outputs.
DEA suffers from the curse of dimensionality, in the sense that the dataset should grow exponentially as the number of inputs and outputs increases, otherwise the efficiency scores are not reliable.
As they have a large number of inputs and outputs, they use the model from \citet{A774} to see which inputs and outputs are redundant for the analysis.
The second test that they employ is an outlier detection test, to prevent mistakes in the self-reported data from distorting the analysis.
The third test checks whether their are efficiency differences between warehouses operating in different industries.\\
The research mentioned above shows that for empirical warehousing datasets, a basic DEA is usually not sufficient, but should be complemented by regressions and statistical tests to account for violation of assumptions and irregularities in the data.
These papers study DEA in the context of warehousing, but use DEA to evaluate the warehouse performance over a relatively long period of time, not to evaluate strategies or rules to solve operational problems or combinations of operational problems.
Some papers do try to solve several operational jointly, or study rules for operational problems separately, but use different techniques.
For example \citet{A729} use ANOVA to analyze storage, batching, zoning and routing policies in a case study, \citet{A775} formulate joint order batching and order picking as a combinatorial optimization problem and solve it using heuristics, \citet{A776} formulate the integrated order batching, sequencing and routing problem as a combinatorial optimization problem that is solved using genetic algorithms and \citet{A441} and \citet{A777} do use simulations to evaluate different policies but do not use DEA to analyze the results.
DEA has been applied to simulations of warehouses or in a similar context. For example, \citet{A648} use simulations and DEA to study vehicle dispatching rules for AGVs in a container terminal, \citet{A745} use simulations and DEA to study design aspects in pick and pass zone picking systems, and \citet{A618} simulate a regular warehouse to study combinations of storage policies, order sequencing rules and routing policies, and use DEA to show the combination that is efficient when the output of handled orders, the service level and the operational costs need to be considered jointly.\\
Using DEA in the context of warehouse simulations has a number of advantages.
The homogeneity assumption is not violated, as for all simulations the warehouse is operating under identical conditions.
Moreover, usually in DEA studies only one datapoint is available for each DMU, one realization of the outputs $y$ for one configuration of the inputs $x$, which means that two DMUs can usually not be compared directly as the values for their inputs were different. \todo{but this is actually making things complicated}
With simulations, the production function of a DMU can be explored further and for all relevant configurations of inputs $x$ realization of outputs $y$ can be created, so that all DMUs can be compared for exactly the same values of inputs $x$.
Moreover, for each DMU the Most Productive Scale Size (MPSS) can be calculated, the values of the inputs for which the average productivity of that DMU is the highest.\\
The DEA set-up for our DEA and simulations is as follows.
Returns to scale are variable and not constant, because there is queueing at the workstations, so for example doubling the number of robots does not double the order throughput.
All possible DMUs are defined by \autoref{eq:policySet}. It is given by the cross product of all path planning ($\mDEASetPathPlanners$), task allocation ($\mDEASetTaskAllocators$), bundle storage ($\mDEASetBundleStoragers$), pod storage ($\mDEASetPodStoragers$), replenishment assignment ($\mDEASetReplenishmentAllocators$) and order assignment mechanisms ($\mDEASetOrderAllocators$).

\begin{equation}\label{eq:policySet}
\Omega := \mDEASetPathPlanners \times \mDEASetTaskAllocators \times \mDEASetBundleStoragers \times \mDEASetPodStoragers \times \mDEASetReplenishmentAllocators \times \mDEASetOrderAllocators = \left\{ \left( \mDEAIndexPathPlanner, \mDEAIndexTaskAllocator, \mDEAIndexBundleStorager, \mDEAIndexPodStorager, \mDEAIndexReplenishmentAllocator, \mDEAIndexOrderAllocator \right) \mid \mDEAIndexPathPlanner \in \mDEASetPathPlanners, \mDEAIndexTaskAllocator \in \mDEASetTaskAllocators, \mDEAIndexBundleStorager \in \mDEASetBundleStoragers, \mDEAIndexPodStorager \in \mDEASetPodStoragers, \mDEAIndexReplenishmentAllocator \in \mDEASetReplenishmentAllocators, \mDEAIndexOrderAllocator \in \mDEASetOrderAllocators \right\}
\end{equation}

The efficiency score of each DMU is determined with the LP denoted by \autoref{eq:deaModelStart} to \ref{eq:deaModelEnd}. The inputs of a DMU are the number of robots used ($\mDEAInBotCount{\mDEADMUIndex}$) and the number of SKUs available ($\mDEAInSKUCount{\mDEADMUIndex}$). As outputs we use the item throughput rate relative to the upper bound of the respective system ($\mDEAOutItemThroughputScore{\mDEADMUIndex}$), the number of pods processed for picking relative to the overall processed pods ($\mDEAOutItemThroughputScore{\mDEADMUIndex}$), the inverse of the average turnover time of the orders ($\mDEAOutTurnoverTime{\mDEADMUIndex}$) and the inverse of the wall time consumed by the DMU ($\mDEAOutDecisionTime{\mDEADMUIndex}$).

\begin{equation}\label{eq:deaModelStart}
\min \theta_{\mDEADMUIndex}
\end{equation}
\begin{align}
\text{s.t.} \sum_{i = 1}^{\left| \Omega \right|} \lambda_{i} \mDEAInBotCount{i} &\le \theta \mDEAInBotCount{\mDEADMUIndex}\\
\sum_{i = 1}^{\left| \Omega \right|} \lambda_{i} \mDEAInSKUCount{i} &\le \theta \mDEAInSKUCount{\mDEADMUIndex}\\
\sum_{i = 1}^{\left| \Omega \right|} \lambda_{i} \mDEAOutItemThroughputScore{i} &\ge \mDEAOutItemThroughputScore{\mDEADMUIndex}\\
\sum_{i = 1}^{\left| \Omega \right|} \lambda_{i} \mDEAOutPickPods{i} &\ge \mDEAOutPickPods{\mDEADMUIndex}\\
\sum_{i = 1}^{\left| \Omega \right|} \lambda_{i} \frac{1}{\mDEAOutTurnoverTime{i}} &\ge \frac{1}{\mDEAOutTurnoverTime{\mDEADMUIndex}}\\
\sum_{i = 1}^{\left| \Omega \right|} \lambda_{i} \frac{1}{\mDEAOutDecisionTime{i}} &\ge \frac{1}{\mDEAOutDecisionTime{\mDEADMUIndex}} \\
\sum_{i = 1}^{\left| \Omega \right|} \lambda_{i} & =1 \label{eq:deaModelEnd}
\end{align}

==> sections/titlepage-elsarticle.tex <==
\begin{frontmatter}

%% Title, authors and addresses

%% use the tnoteref command within \title for footnotes;
%% use the tnotetext command for the associated footnote;
%% use the fnref command within \author or \address for footnotes;
%% use the fntext command for the associated footnote;
%% use the corref command within \author for corresponding author footnotes;
%% use the cortext command for the associated footnote;
%% use the ead command for the email address,
%% and the form \ead[url] for the home page:
%%
%% \title{Title\tnoteref{label1}}
%% \tnotetext[label1]{}
%% \author{Name\corref{cor1}\fnref{label2}}
%% \ead{email address}
%% \ead[url]{home page}
%% \fntext[label2]{}
%% \cortext[cor1]{}
%% \address{Address\fnref{label3}}
%% \fntext[label3]{}

%\dochead{}
%% Use \dochead if there is an article header, e.g. \dochead{Short communication}
%% \dochead can also be used to include a conference title, if directed by the editors
%% e.g. \dochead{17th International Conference on Dynamical Processes in Excited States of Solids}

\title{Decision Rules for Robotic Mobile Fulfillment Systems}

%% use optional labels to link authors explicitly to addresses:
\author[label1]{M. Merschformann\corref{cor1}}
\author[label2]{T. Lamballais}
\author[label2]{M.B.M. De Koster}
\author[label1]{L. Suhl}
\cortext[cor1]{Corresponding author}
\address[label1]{DS\&OR Lab, Paderborn University, Warburger Str. 100, 33098, Paderborn, Germany}
\address[label2]{Rotterdam School of Management, Erasmus University, PO Box 1738, Rotterdam 3000 DR, The Netherlands}


\begin{abstract}
The Robotic Mobile Fulfillment Systems (RMFS) is a new type of robotized, parts-to-picker material handling system, designed especially for e-commerce warehouses.
Robots bring movable shelves, called pods, to workstations where inventory is put on or removed from the pods.
This paper simulates both the pick and replenishment process and studies the order assignment, pod selection and pod storage assignment problems by evaluating 
multiple decision rules per problem.
The discrete event simulation uses realistic robot movements and keeps track of every unit of inventory on every pod.
We analyze seven performance measures, e.g. throughput capacity and order due time, and find that the unit throughput is strongly correlated with the 
other performance measures.
We vary the number of robots, the number of pick stations, the number of SKUs (stock keeping units), the order size and whether returns need processing or not.
The decision rules for pick order assignment have a strong impact on the unit throughput rate. 
This is not the case for replenishment order assignment, pod selection and pod storage.
Furthermore, for warehouses with a large number of SKUs, more robots are needed for a high unit throughput rate, even if the number of pods and the dimensions of the storage area remain the same.
Lastly, processing return orders only affects the unit throughput rate for warehouse with a large number of SKUs and large pick orders. 
\end{abstract}

\begin{keyword}

Warehouse Control \sep Simulation \sep Robotic Mobile Fulfillment System \sep Parts-to-Picker System

%% keywords here, in the form: keyword \sep keyword

%% PACS codes here, in the form: \PACS code \sep code

%% MSC codes here, in the form: \MSC code \sep code
%% or \MSC[2008] code \sep code (2000 is the default)

\end{keyword}

\end{frontmatter}
